Statistical Inference and A/B Testing in Fisher Markets and Paced Auctions

We initiate the study of statistical inference and A/B testing for two market equilibrium models: linear Fisher market (LFM) equilibrium and first-price pacing equilibrium (FPPE). LFM arises from fair resource allocation systems such as allocation of food to food banks and notification opportunities to different types of notifications. For LFM, we assume that the data observed is captured by the classical finite-dimensional Fisher market equilibrium, and its steady-state behavior is modeled by a continuous limit Fisher market. The second type of equilibrium we study, FPPE, arises from internet advertising where advertisers are constrained by budgets and advertising opportunities are sold via first-price auctions. For platforms that use pacing-based methods to smooth out the spending of advertisers, FPPE provides a hindsight-optimal configuration of the pacing method. We propose a statistical framework for the FPPE model, in which a continuous limit FPPE models the steady-state behavior of the auction platform, and a finite FPPE provides the data to estimate primitives of the limit FPPE. Both LFM and FPPE have an Eisenberg-Gale convex program characterization, the pillar upon which we derive our statistical theory. We start by deriving basic convergence results for the finite market to the limit market. We then derive asymptotic distributions, and construct confidence intervals. Furthermore, we establish the asymptotic local minimax optimality of estimation based on finite markets. We then show that the theory can be used for conducting statistically valid A/B testing on auction platforms. Synthetic and semi-synthetic experiments verify the validity and practicality of our theory.

==> old_fppe_results.tex <==
\section{Statistical Results for FPPE}

Next we study statistical inference questions for the FPPE model.
Since FPPE is characterized by an EG-style program similar to that of LFM, many of the results for FPPE are similar to those for LFM. However, an important difference is that the FPPE model has constraints on the pacing multipliers, which makes the asymptotic theory more involved.
As for LFM, we assume that we observe a finite auction 
market $\oFPPE(b,v,1/t, \gamma)$ with $\gamma$ being $t$ i.i.d. draws from $s(\cdot)$, and we use it to estimate quantities from the limit market $\FPPE(b,v,s,\Theta)$.
In FPPE we mainly focus on the revenue of the limit market, and for the same reason as in LFM, since FPPE is characterized by EG program with optimizing variable being the pacing multiplier, we also present results for $\b$.
Similarly to the LFM case, one could use results for $\b$ to derive estimators for buyer utilities.
% In \cref{sec:fppe_basic}
% we provide strong consistency and convergence rates for revenue and $\b$.
% In \cref{sec:fppe_asym} we present asymptotic distributions. 
% Compared with LFM, the asymptotic theory for FPPE is more involved due the present of constraints in its EG program.
% In \cref{sec:fppe_inference} we estimate the asymptotic variances.


\subsection{Basic Convergence Properties}
\label{sec:fppe_basic}
Since FPPE has a similar convex program characterization as LFM, strong consistency and convergence rate results can be derived using similar ideas.

\begin{theorem}\label{thm:fppe_as_convergence}
    We have $\betagam \toas \betast$,
    and $\REVgam \toas \REVst$. Proof in Appendix~\ref{sec:proof:thm:fppe_as_convergence}.
\end{theorem}

We complement the strong consistency result with the following rate results. They are derived using a discretization argument.
\begin{theorem}
    \label{thm:rev_convergence}
    It holds that
    $ \| \betagam - \betast\|_2
    = \tilde O_p(\frac{\sqrt{n} (\vbar + 2\nubar n + 1)}{\ubar{b} \sqrt t})
    $
    and
    $ | \REV^\gam - \REV^* | = 
        \tilde{O}_p
        (\frac{\vbar \sqrt{n} (\vbar + 2\nubar n + 1 ) }{ \ubar{b} }\frac{1}{\sqrt{t}}).$
    Proof in Appendix~\ref{sec:proof:thm:rev_convergence}.
\end{theorem}

The above bounds hold for a broad class of limit FPPE models and may be loose for a particular model. 
In \cref{sec:fppe_asym}, we show that for buyers $i \in \{ i:\betasti = 1\}$, their pacing multipliers converge at a rate faster than $ \tilde O_p(1/\sqrt t)$.



\subsection{Asymptotics of FPPE}
\label{sec:fppe_asym}

As in LFM, our statistical inference results require the limit market to behave smoothly around the optimal pacing multipliers $\betast$.
To that end, we will assume \cref{as:smo} as in LFM.
Similar to LFM, under \cref{as:smo}, the equilibrium allocation $\xst$ is unique and must be pure. 
Again we can define 
\begin{align}
    \label{eq:def:must}
     \must (\t) = [x^*_1(\t) v_1(\t), \dots, x^*_n(\t) v_n (\t)]\tp\; .
\end{align}
Under \cref{as:smo}, the equilibrium allocation $\xst$ is unique, so $\must(\cdot)$ is also unique. 
Moreover, $\must(\t) = \nabla f(\t, \betast)$, 
and $ (\betast) \tp \must(\t) = \pst(\t)$ (the set of nondifferentiable points has measure zero, and thus we can ignore such points). 
% CK: the below was already defined in the previous sentence.
Also let 
\begin{align}
    \label{eq:def:mubarst}
    \mubarst = \int \must s \dt \in \Rnp
\end{align}
to denote the utility from items. 
Note that in the FPPE model, buyers' utility consists of two parts: utility from items and leftover budgets.
In FPPE, the pacing multipliers relate budgets and utilities via \citep{conitzer2022pacing} 
\begin{align} \label{eq:beta_u_relation_fppe}
    \mubarsti + \deltasti = b_i/ \betasti \;.
\end{align}

In the unconstrained case, classical $M$-estimation theory says that, under regularity conditions, an $M$-estimator is asymptotically normal with covariance matrix $\cH\inv  \var(\text{gradient}) \cH\inv$ \citep[Chap.\ 5]{van2000asymptotic}. However, in the case of FPPE which is characterized by a constrained convex problem, the Hessian matrix needs to be adjusted to take into account the geometry of the constraint set $B=(0,1]^n$ at the optimum $\betast$.
We let $\cP \defeq \Diag( \indi( \betasti < 1) )$ be an ``indicator matrix'' of buyers whose $\betasti < 1$, and define the projected Hessian 
\begin{align}
    \label{def:cHB}
    \cH_B \defeq \cP \cH \cP \;.
\end{align}
It will be shown that the asymptotic variance of $\betagam$ is $\cH_B\pinv \var(\text{gradient}) \cH_B\pinv$ and the ``gradient" is exactly $\must$.

\begin{assumption}[\textsf{\scriptsize{SCS}}] 
    \label{as:scs} Strict complementary slackness holds:
     $\betasti = 1$ implies  $\delta^*_i  > 0$.
\end{assumption}

\cref{as:scs} can be viewed as a non-degeneracy condition from a convex programming perspective, since $\delta_i$ corresponds to a Lagrange multiplier on $\beta_i \leq 1$.
From a market perpective, \cref{as:scs} requires that if a buyer's bids are not paced ($\betasti = 1$), then their leftover budget $\delta^* _i$ must be strictly positive.
This can again be seen as a market-based non-degeneracy condition: if $\deltasti=0$ then the budget constraint of buyer $i$ is binding, yet $\betasti=1$ would imply that they have no use for additional budget.
% This is a mild requirement; the only way for it to be violated would be if 
% if one bids exactly how much he values the item without scaling them down, it shows that her budget is superfluous for winning her desired items through the sequence of auctions. The situation where such a buyer happens to have no budget left is an edge case.
If \cref{as:scs} fails, one could slightly increase the budgets of buyers for which \cref{as:scs} fails, i.e., those who do not pace yet have exactly zero leftover budget, and obtain a market instance with the same equilibrium, but where \cref{as:scs} holds.

From a technical viewpoint, \cref{as:scs} is a stronger form of first-order optimality.  
Note $\nabla H(\betast) = -\deltast$ (cf.\ \cref{lm:fppe_relation}). 
The usual first-order optimality condition is 
\begin{align}
    - \nabla H(\betast) \in \cN_B(\betast) \;,
    \label{eq:usual_foc}
\end{align}
where $\cN_B(\beta) = \prod_{i=1}^n J_i(\beta)$ is the normal cone with $J_i (\beta)= [0,\infty)$
if $\betai = 1$ and $J_i (\beta)= \{0\}$ if $\betai < 1$ for $\beta \in \Rnpp$.
Then \cref{eq:usual_foc} translates to the condition that $\betasti = 1$ implies $\deltasti \geq 0$. 
On the other hand, when written in terms of the normal cone, 
\cref{as:scs} is equivalent to $$- \nabla H(\betast) \in \relint ( \cN_B(\betast) ) \; .
\footnote{
    The relative interior of a set is $\relint(S)\defeq\{x \in S:$ there exists $\epsilon>0$ such that $N_\epsilon(x) \cap \operatorname{aff}(S) \subseteq S \}$ where $\operatorname{aff}(S)$ is the affine hull of $S$, and $N_\epsilon(x)$ is a ball of radius $\epsilon$ centered on $x$. %For example, the interior of a line segment on $\R^2$ is empty, but its relative interior is the line segment without its endpoints.
}$$
Given that $ \relint ( \cN_B(\betast) ) \subset \cN_B(\betast) $, \cref{as:scs} is obviously a stronger form of first-order condition. The \cref{as:scs} condition is commonly seen in the study of statistical properties of constrained $M$-estimators (\citealt[Assumption B]{duchi2021asymptotic} and \citealt{shapiro1989asymptotic}). In the proof of \cref{thm:clt}, \cref{as:scs} forces the critical cone to reduce to a hyperplane and thus ensures asymptotic normality of the estimates.
Without \cref{as:scs}, the asymptotic distribution of $\betagam$ could be non-normal.
% \ck{critical cone is only defined in appendix. Not sure if it's possible to give a high-level idea of what it is here?}


\subsubsection{Asymptotic Normality}
We now show that the observed pacing multipliers $\betagam$ and the observed revenue $\REV^\gamma$ are asymptotically normal.
Define the \emph{influence functions} 
\begin{equation} \label{eq:def_inf_func}
    \begin{aligned}
    D_\beta(\theta) & \defeq - (\cH_B)^\dagger (\must(\theta) - \mubarst) ,
    \\
    D_\REV(\theta) & \defeq \pst(\theta) - \REV^* + (\mubarst) \tp D_\beta(\theta).
    \end{aligned}
\end{equation}
Recall $\must$ is defined in \cref{eq:def:must}, $\mubarst$ in \cref{eq:def:mubarst}, $\cH_B$ in \cref{def:cHB}.
And note $\E[D_\beta] = 0$ and $\E[D_\REV] = 0$.

\begin{theorem} 
    \label{thm:clt}
    If
    \cref{as:smo,as:scs} hold, then 
    \begin{align*}
        &\sqrt{t}(\betagam - \betast) =  \frac1\roott \sumtau D_\beta (\thetau) + o_p(1) \; ,
        \\
        &\sqrt{t} (\REV^\gam - \REV^*) = \frac1\roott \sumtau D_\REV(\thetau) + o_p(1)  \;.
    \end{align*}
    Consequently, $ \sqrt{t}(\betagam - \betast )$ and $\sqrt {t} (\REV^\gamma - \REV^*) $
    are asymptotically normal with means zero and variances $\Sigma_\beta\defeq \E[D_\beta D_\beta\tp ] =  (\cH_B)\pinv \var(\must) (\cH_B)\pinv$ and $\sigma^2_\REV \defeq \E[D_\REV (\theta)^2]$. 
    Proof in Appendix~\ref{sec:proof:thm:clt}.
\end{theorem}


The functions $D_\beta$ and $D_\REV$ are called the {influence functions} of the estimates $\betagam$ and $\REV^\gam$ because they measure the change in the estimates caused by adding a new item to the market (asymptotically).

\cref{thm:clt} implies fast convergence rate of $\betagami$ for $i \in \{ \betasti =1\}$. 
To see this, we 
suppose wlog.\ that $I_= = [k]$, i.e. the  first $k$ buyers are the ones with $\beta_i=1$.
Then the pseudo-inverse of the projected Hessian $(\cH_B )\pinv = \Diag(0_{k\times k} , (\cH_{<})\inv )$ where $\cH_{<}$ is the lower right $(n-k)\times(n-k)$ block of $\cH $ corresponding to $I_<$. 
Consequently, the upper $k$ diagonal entries of $\Sigma_\beta$ are zeros. 
This result shows that the constraint set $B$ ``improves'' the covariance by zeroing out the entries in $\Sigma_\b$ corresponding to the active constraints $I_=$.
Consequently, 
$ \sqrt{t} (\betagami - \betasti)$ is of order $o_p(1)$ for $i \in I_=$, and thus converging faster than the usual $O_p(1)$ rate.
The fast rate phenomenon is empirically investigated in \cref{sec:exp_fast_rate}. 

The practical implication is the following.
By \cref{as:scs} we have $I_= = \{i: \betasti = 1\}= \{ i: \deltasti > 0\}$, i.e., $I_=$ is the set of buyers who are not budget constrained, and $\Ic = \{i:\betasti < 1\} = \{ i: \deltasti = 0\} $, i.e., $\Ic\,$ is the set of buyers who exhaust their budgets. \footnote{Without \cref{as:scs}, it only holds $ \{i:\betasti < 1\} \subset \{i:\deltasti = 0\}$ and $\{i:\deltasti > 0 \}\subset \{i:\betasti = 1\}$ by complementary slackness.}
In the context of first-price auctions,
the fast rate $o_p(t^{-1/2})$ implies that the platform can identify  which buyers are budget constrained even when the finite market is small.

The proof of \cref{thm:clt} proceeds by showing that FPPE satisfy a set of regularity conditions that are sufficient for asymptotic normality~\citep[Theorem 3.3]{shapiro1989asymptotic}; the conditions are stated in \cref{thm:the_shapiro_thm} in the appendix. Maybe the hardest condition to verify is the so called stochastic equicontinuity condition (\cref{it:stoc_equic}), which we establish with tools from the empirical process literature. 
In particular, we show that the class of functions, parameterized by a pacing multiplier vector $\beta$, that map each item to its corresponding first-price auction allocation under the given $\beta$, is a VC-subgraph class. This in turn implies stochastic equicontinuity. 
\cref{as:scs} is used to ensure normality of the limit distribution.

Finally, we remark that the CLT result for revenue holds true 
even if $I_= = \emptyset$, i.e., $\betasti < 1$ for all $i$.
In this case, the limit theorem writes 
$\sqrt t (\REVgam - \REVst) \tod N(0,0)$, equivalent to $\sqrt t (\REVgam - \REVst) = o_p(1)$.
We briefly explain why this is expected when all buyers are paced.
If $\betagami < 1$ for all $i$, then all buyers' budgets are exhausted in the observed FPPE, and so we have
$
    \REVgam = \REVst = \sumiton b_i$. 
By the convergence $\betagam \toprob \betast$, we know that 
$\REVgam = \REVst$ with high probability for all large~$t$ if $I_==\emptyset$.
In that case, it must be that the asymptotic variance of revenue equals zero.
Our result covers this case because one can show $\sigma\sq_\REV = 0$ using $\cH \betast = \mubarst$ if $I_= = \emptyset$ (\cref{lm:fppe_relation}), and $(\betast)\tp \must(\t) = \pst(\t)$.
A more general relation between $D_\REV$ and prices is given below.

\new{
\begin{claim} \label{cl:rev_influence_function}
    Let \cref{as:smo} hold. Let $\tilde p^*(\t) =  p^*(\t) \indi\{ \max_{i \in I_=} \betasti \vithe = \max_{i \in [n]} \betasti \vithe \} $  if $I_= \neq \emptyset$ and $\tilde p ^*(\t) = 0$ otherwise. 
    Then $D_\REV(\t) = \tilde p^* (\t) -\E[\tilde p^*]$. 
    Proof in \cref{sec:proof:cl:rev_influence_function}
\end{claim}
}

In an FPPE individual utilities and Nash social welfare can be similarly defined. 
By applying the delta method and the results in \cref{thm:clt}, we can derive asymptotic distributions for individual utilities $\ugam$, leftover budget $\deltagam$ and Nash social welfare, since they are smooth functions of $\beta$. See \cref{sec:full:cor:clt_u_and_nsw} for more details.

% \begin{corollary}
%     \label{cor:clt_u_and_nsw}
%     Under the same conditions as \cref{thm:clt},
%        $\sqrt{t} (\ugam - \ust) $, $\sqrt t(\deltagam - \deltast)$ and $\sqrt{t}(\NSW^\gam - \NSW^*) $
%        are asymptotically normal with means zero and 
% (co)variances defined in \cref{sec:full:cor:clt_u_and_nsw}.
% \end{corollary}


\subsubsection{Asymptotic Local Minimax Optimality}

Given the asymptotic distributions for $\beta, u, \NSW$ and $\REV$, we will show that the observed FPPE estimates are optimal in an asymptotic local minimax sense.
Recall in \cref{sec:perturb_supply} we have defined the perturbed supply family $G_d$ of dimension $d$ with perturbation $(\alpha,g)$.

\paragraph{Asymptotic local minimax optimality for $\beta$.}
We first focus on estimation of pacing multipliers.\
For a given perturbation ${(\alpha,g)}$, we let $\betast_{\alpha,g}$, $\pst_{\alpha,g}$ and $\REVst_{\alpha,g}$ be the limit FPPE pacing multiplier, price and revenue under supply distribution $s_{\alpha,g}$.
Clearly $\betast = \betast_{0,g}$ for any $g$ and similarly for $\pst_{\alpha,g}$ and $\REV_{\alpha, g}$.
Let $L:\Rn \to \R$ be any symmetric quasi-convex loss. 
\footnote{A function is quasi-convex if its sublevel sets are convex.}
In asymptotic local minimax theory we are interested in the local asymptotic risk: given a sequence of estimators $\{ \hat \beta_t: \Theta^t \to \Rn \}_t$, 

\begin{equation*}
\LAR_\beta (\{\hat \beta_t\}_t )  \defeq 
    {\sup_{ g\in G_d, d\in \mathbb{N}}
    \lim_{c\to \infty}
    \liminf_{t \to \infty}
    \sup_{\|\alpha\|_2\leq \frac{c}{\sqrt t}}
    \E_{s_{\alpha,g}^{\otimes t}}[L(\sqrt{t} (\hat \beta_t - \betast_{\alpha,g} ))] } \;.
\end{equation*}
As an immediate application of Theorem 1 from \citet{duchi2021asymptotic}, it holds that 
\begin{align*}
    \inf_{ \{\hat \beta_t\}_t }  \LAR_\beta (\{\hat \beta_t\}_t )  \geq \E[L(\cN( 0, (\cH_B)\pinv \var(\must) (\cH_B)\pinv))] \; . 
\end{align*}
where the expectation is taken w.r.t.\ a normal specified above.
Moreover, the lower bound is achieved by the observed FPPE pacing multipliers $\betagam$ according to the CLT result in \cref{thm:clt}.

\paragraph{Asymptotic local minimax optimality for revenue estimation.}
For pacing multipliers, the result is a direct application of the perturbation result from \citet{duchi2021asymptotic}. The result for revenue estimation is more involved.
Given a symmetric quasi-convex loss $L:\R\to\R$, we define the local asymptotic risk for any procedure $\{\hat r _t : \Theta^t \to \R\}$ that aims to estimate the revenue: 
\begin{align*} \hspace{-.2cm}
\LAR_\REV ( \{\hat r_t \}) \defeq
    \sup_{ g\in G_d, d\in \mathbb{N}}
    \lim_{c\to \infty}
    \liminf_{t \to \infty}
    \sup_{\|\alpha\|_2\leq \frac{c}{\sqrt t}}
    \E_{s_{\alpha,g} ^{\otimes t}}[L(\sqrt{t} (\hat r_t  - \REVst_{\alpha,g} ))] \;. 
\end{align*} 
\begin{theorem}[Asymptotic local minimaxity for revenue]
    \label{thm:rev_localopt}
   If \cref{as:smo,as:scs} hold, then 
    \begin{align*}
       \inf_{ \{\hat r_t\}} \LAR_\REV ( \{\hat r_t \}) \geq \E[L(\cN(0, \sigma\sq_\REV))] \;.
    \end{align*} 
\end{theorem}

Proof in Appendix~\ref{sec:proof:rev_local_asym_risk}. In the proof we calculate the derivative 
of revenue w.r.t.\ $\alpha$, which in turn uses 
a perturbation result for constrained convex programs from \citet{duchi2021asymptotic,shapiro1989asymptotic}.
Again, the lower bound is achieved by the observed FPPE revenue $\REVgam$ according to the CLT result in \cref{thm:clt}.
Similar optimality statements can be made for $u$ and $\NSW$ by finding the corresponding derivative expressions.


\subsection{Variance Estimation and Inference}
\label{sec:fppe_inference}

In order to perform inference, we need to construct estimators for the influence functions \cref{eq:def_inf_func}. In turn, this requires estimators for 
the projected Hessian $\cH_B$ (\cref{def:cHB}) and the variance of the utility map $\must$ (\cref{eq:def:must}).

\textbf{The Hessian.}
Given a sequence of smoothing parameters $\varepsilon_t = o(1)$, we estimate the projection matrix $\cP$ by 
$
    \hat \cP \defeq \Diag(\indi(\betagami < 1 - \varepsilon_t )) \;.
$
For the same sequence $\varepsilon_t$, we introduce a numerical difference estimator $\hat \cH$ for the Hessian matrix $\cH$, whose $(i,j)$-th entry is
\begin{align}
    \label{eq:def:hessian_estimate}
    \hat{\cH}_{i j}\defeq[H_t(\betagam_{++})-H_t(\betagam_{+-})
     -H_t(\betagam_{-+}) 
    +H_t(\betagam_{--})] / 4 \varepsilon_t^2 
\end{align}  
with 
$\betagam_{\pm \pm} \defeq  \betagam \pm e_i \varepsilon_t \pm e_j \varepsilon_t$,
and $H_t$ is defined in \cref{eq:def_pop_eg}. Finally, $\hat \cH_B = \hat \cP \hat \cH \hat \cP$ is the estimator of $\cH_B$. 


\textbf{The term $\cov(\must)$.}
Let $\xgam = (\xitau)_{i,\tau}$ and price $\pgam = [p^1, \dots, p ^ t ] \tp $ be the allocation and prices in the finite FPPE.
Mimicking \cref{eq:def:must,eq:def:mubarst}, define the finite sample analogues
\begin{align}
   \mu^\tau = [x_1^{\tau} v_1^\tau, \dots, x_n^{\tau} v_n^\tau]\tp, \;\quad \bar \mu= \frac1t \sumtau \mutau \;.
\end{align}
Recall $\REVgam = \frac1t \sumtau \ptau$.
Then we define the following influence function estimators
\begin{align*}
    \hat D_\beta^\tau  \defeq - (\hat \cH_B)\pinv (\mutau- \mubar) \;,
    \quad
    \hat D _\REV ^\tau \defeq \ptau - \REV^\gamma + (\mubar) \tp\hat D_\beta^\tau \;.
\end{align*}
\todo{new formula for revenue D}
% which estiamte the influence functions $D_\beta$ and $D_\REV$ evaluated at item $\thetau$.
Given that the asymptotic variance of $\betagam$ (resp.\ $\REVgam$) is 
$\E[D_\beta D_\beta \tp]$ (resp.\ $\E[D_\REV\sq]$), plug-in estimators for the (co)variance are naturally
\begin{align}
    \hat \Sigma_\beta \defeq \frac{1}{t} \sumtau \hat D_\beta^\tau  (\hat D_\beta^\tau )\tp \; , \;\;
    \hat \sigma \sq_\REV \defeq \frac{1}{t} \sumtau (\hat D_\REV ^\tau)\sq \; .
    \label{eq:plugin variance}
\end{align}
For any $\alpha \in (0,1)$, the $(1-\alpha)$-confidence regions for $\betast$ and $\REVst$ are 
\begin{align}
   & \CR_\beta\defeq \betagam + (\chi_{n, \alpha} / \sqrt{t})\hat \Sigma_\beta^{1/2} \B \; ,\label{eq:beta CI}
    \\ 
   & \CI_\REV \defeq\Big[\REVgam\pm z_{\alpha/2}  \hat \sigma_{\REV}/\sqrt t\Big] \; .
   \label{eq:rev_variance}
\end{align} 
where $\chi_{n,\alpha}$ is the $(1-\alpha)$-th quantile of a chi-square distribution with degree $n$, $\B$ is the unit ball in $\Rn$, and $z_{\alpha/2}$ is the $(1-\frac{\alpha}{2})$-th quantile of a standard normal distribution.
The coverage rate of $\CI_\REV$ is empirically verified in \cref{sec:exp_rev_coverage}.
\begin{theorem}
    \label{thm:variance_estimation}
    Under the conditions of \cref{thm:clt}, 
    let $\varepsilon_t \sqrt{t}\to \infty$ and $\varepsilon_t = o(1)$. 
    Then $\hat \Sigma_\beta \toprob \Sigma_\beta$ and $\hat \sigma_\REV \sq \toprob \sigma_\REV \sq$. 
    Consequently, for any $\alpha \in (0,1)$,
    $\P (\betast \in \CR_\beta ) \to 1-\alpha$ and $\P(\REVst \in \CI_\REV ) \to 1-\alpha$. 
    Proof in Appendix~\ref{sec:proof:thm:variance_estimation}.
\end{theorem}
The theorem suggests choosing smoothing parameter $\varepsilon_t = t^{- d}$ for $0 < d < \frac12$. \cref{sec:exp_hessain} studies how the choice of $d$ affects the Hessian estimation numerically.
% Variance estimators for $u$, $\delta$ and $\NSW$ can be constructed similarly. 
% $
%      \hat \Sigma_u \defeq \allowbreak \Diag{({b_i}/({\betagami})\sq)} \allowbreak \hat  \Sigma_\beta  \allowbreak    \Diag({b_i}/({\betagami})\sq) \text{ and }
%      \hat \sigma^2_\NSW\defeq\Vec(b_i/\betagami)\tp \allowbreak \hat\Sigma_\beta \allowbreak\Vec(b_i / \betagami) \;.
% $
% Their consistency is ensured by Slutsky's theorem. The corresponding confidence region/interval are $ \CR_u \defeq \ugam + (\chi_{n, \alpha} / \sqrt{t})\hat \Sigma_u^{1/2} \B$ and 
% $ \CI_\NSW \defeq[\NSWgam\pm z_{\alpha/2}  \hat \sigma_{\NSW}/\sqrt t] $. 
\subsection{Application: A/B Testing in First-Price Auction Platforms}
\label{sec:ab testing}

Consider an auction market with $n$ buyers with a continuum of items $\Theta$ with supply function $s$.
Now suppose that we are interested in the effect of deploying some new technology (e.g. new machine learning models for estimating click-through rates in the ad auction setting).
To model treatment application we introduce the \emph{potential value functions}
$$ \hspace{-.2cm} v(0) \defeq (v_1(0,\cdot),\dots, v_n(0,\cdot)),\;v(1)\defeq (v_1(1,\cdot),\dots, v_n(1,\cdot)).$$
If item $\theta$ is exposed to treatment $w \in \{0,1\}$, then its value to buyer $i$ will be $v_i(w,\theta)$. %Let $s$ is the supply distribution of items.


Suppose we are interested in estimating the change in the auction market when treatment 1 is deployed to the entire item set $\Theta$. 
In this section we describe how to do this using A/B testing, specifically for estimating the treatment effect on revenue. %Analogous results can be readily developed for pacing multipliers using \cref{eq:beta CI}.   
Formally, we wish to look at the difference in revenues between the markets 
$$
    \FPPE(b, v(0), s) \text{ and }  \FPPE(b,v(1), s),
$$
where $\FPPE(b, v(0), s)$ is the market with treatment 1, and $\FPPE(b,v(1), s)$ is the one with treatment 0. %, both defined in \cref{def:limit_fppe}.
The treatment effects on revenue is defined as $$\tau_{\REV} \defeq \REVst(1) - \REVst(0)\;,$$
where $\REVst(w)$ is revenue in the equilibrium $\FPPE(b,v(w), s)$.

We will refer to the experiment design as \emph{budget splitting with item randomization}.
The design works in two steps, and closely mirrors how A/B testing is conducted at large tech companies.

\textbf{Step 1. Budget splitting.}
    We create two markets, and every buyer is replicated in each market.
    For each buyer $i$ we allocate $\pi b_i$ of their budget to the market with treatment $w=1$, and the remaining budget, $(1-\pi)b_i$, to the market with treatment $w=0$.
    Each buyer's budget is managed separately in each market.

\textbf{Step 2. Item randomization.}
Let $(\theta^1,\theta^2,\dots)$ be i.i.d.\ draws from the supply distribution $s$.
For each sampled item, it is applied treatment $1$ with probability $\pi$ and treatment $0$ with probability $1-\pi$.  
The total A/B testing horizon is $t$. When the end of the horizon is reached, two observed FPPEs are formed. Each item has a supply of $\pi/t_1$ in the 1-treated market and $(1-\pi)/t_0$ in the 0-treated market. The $1/t_1$ is the scaling required for our CLTs and the $\pi$ factor ensures the budget-supply ratio agrees with the limit market; 
due to FPPE scale-invariance, we could equivalently rescale budgets.

Let $t_0$ be the number of $0$-treated items, and $t_1$ be the number of $1$-treated items. Conditional on the total number of items $t=t_1 + t_0$, the random variable $t_1$ is a binomial random variable with mean $\pi t$. Let $\gamma(0) = (\theta^{1,1},\dots, \theta^{1,t_1})$ be the set of $0$-treated items, and similarly $\gamma(1) = (\theta^{0,1},\dots, \theta^{0,t_0})$.
The total item set $\gamma = \gamma(0) \cup \gamma(1)$. 
The observables in the described A/B testing experiment are 
$$ \hspace{-.1cm}
\oFPPE \big(\pi b, v(1), \tfrac{\pi}{t_1}, \gamma(1)  \big),\; 
    \oFPPE \big( (1-\pi ) b,  v(0), \tfrac{1-\pi}{t_0}, \gamma(0)\big ), $$
both defined in \cref{def:finite_fppe}.
Let $\REVgam(w)$ denote the observed revenue in the $w$-treated market.
The estimator of the treatment effect on revenue is 
$$
     \hat \tau_{\REV} \defeq \REVgam(1) - \REVgam(0).$$ 

 
For fixed $(b, s)$, the variance $\sigma\sq_\REV$ in \cref{thm:clt} is a functional of the value functions. We will use $\sigma\sq_\REV(w)$ to represent the revenue variance in the equilibrium $\FPPE(b,v(w), s)$.
Each variance can be estimated using \cref{eq:plugin variance}.

\begin{theorem}[Revenue treatment effects CLT]
    \label{thm:clt_ab_testing}
    Suppose \cref{as:smo} and \cref{as:scs} hold in the limit markets $\FPPE(b,v(1),s)$ and $\FPPE(b,v(0),s)$. Then 
 $\sqrt{t} (\hat \tau_\REV - \tau_\REV) \tod\cN\allowbreak \big(0, \frac{ \sigma\sq_\REV(1)}{\pi} \allowbreak + \allowbreak\frac{ \sigma\sq_\REV(0)}{(1-\pi)} \big) .$
Proof in Appendix~\ref{sec:proof:thm:clt_ab_testing}.
\end{theorem}

Based on the theorem, an A/B testing procedure is the following.
Compute the revenue variance as \cref{eq:plugin variance} for each market, obtaining $ \hat \sigma\sq_\REV(1)$ and $ \hat \sigma\sq_\REV(0)$, and form the confidence interval
\begin{align}
    \hat \tau_\REV \pm z_{\alpha/2} \bigg( \frac{ \hat \sigma\sq_\REV(1)}{\pi} \allowbreak + \allowbreak\frac{ \hat \sigma\sq_\REV(0)}{(1-\pi)}  \bigg).
    \label{eq:ab_rev_ci}
\end{align}
If zero is on the left (resp.\ right) of the CI, we conclude that the new feature increases (resp.\ decreases) revenue with $(1-\alpha)\times 100\%$ confidence. 
If zero is in the interval, the effect is undecided.
See \cref{sec:experiment_abtest} for a semi-synthetic study verifying the validity of this procedure.



==> tbl_rev_coverage_with_naive.tex <==
\begin{table}[ht]
\caption{Coverage of revenue CI. $\alpha$ = proportion of $\beta_i = 1$, $d$ is the exponent in finite difference stepsize $\epsilon_t = t^{-d}$.}
\label{tbl:rev_coverage}
\begin{tabular}{lllllllllll}
\toprule
 & buyers & \multicolumn{3}{r}{20} & \multicolumn{3}{r}{50} & \multicolumn{3}{r}{80} \\ \midrule
 & $\alpha$ & 0.00 & 0.10 & 0.20 & 0.00 & 0.10 & 0.20 & 0.00 & 0.10 & 0.20 \\ \midrule
\midrule $d$ & items &  &  &  &  &  &  &  &  &  \\ \midrule
\midrule
\multirow[t]{2}{*}{0.40} & 400 & \makecell{1.0(0.27)\\n:1.0(0.30)} & \makecell{0.85(0.33)\\n:0.87(0.33)} & \makecell{0.92(0.47)\\n:0.9(0.46)} & \makecell{1.0(0.34)\\n:1.0(0.36)} & \makecell{0.91(0.50)\\n:0.86(0.50)} & \makecell{0.93(0.52)\\n:0.88(0.52)} & \makecell{1.0(0.30)\\n:1.0(0.31)} & \makecell{0.9(0.51)\\n:0.92(0.52)} & \makecell{0.88(0.55)\\n:0.91(0.54)} \\ \midrule
 & 600 & \makecell{1.0(0.22)\\n:1.0(0.25)} & \makecell{0.86(0.27)\\n:0.84(0.27)} & \makecell{0.91(0.38)\\n:0.87(0.39)} & \makecell{1.0(0.28)\\n:1.0(0.29)} & \makecell{0.83(0.41)\\n:0.87(0.41)} & \makecell{0.9(0.42)\\n:0.92(0.43)} & \makecell{1.0(0.24)\\n:1.0(0.25)} & \makecell{0.91(0.42)\\n:0.86(0.42)} & \makecell{0.8(0.44)\\n:0.95(0.44)} \\ \midrule
\cline{1-11}
\multirow[t]{2}{*}{0.33} & 400 & \makecell{1.0(0.27)\\n:1.0(0.30)} & \makecell{0.83(0.32)\\n:0.86(0.33)} & \makecell{0.84(0.47)\\n:0.87(0.47)} & \makecell{1.0(0.34)\\n:1.0(0.36)} & \makecell{0.93(0.50)\\n:0.92(0.49)} & \makecell{0.91(0.52)\\n:0.89(0.52)} & \makecell{1.0(0.29)\\n:1.0(0.31)} & \makecell{0.89(0.51)\\n:0.9(0.51)} & \makecell{0.89(0.55)\\n:0.9(0.54)} \\ \midrule
 & 600 & \makecell{1.0(0.22)\\n:1.0(0.25)} & \makecell{0.81(0.27)\\n:0.76(0.27)} & \makecell{0.83(0.38)\\n:0.92(0.38)} & \makecell{1.0(0.28)\\n:1.0(0.29)} & \makecell{0.9(0.41)\\n:0.86(0.40)} & \makecell{0.89(0.42)\\n:0.88(0.42)} & \makecell{1.0(0.24)\\n:1.0(0.25)} & \makecell{0.87(0.42)\\n:0.85(0.42)} & \makecell{0.94(0.44)\\n:0.92(0.45)} \\ \midrule
\cline{1-11}
\multirow[t]{2}{*}{0.17} & 400 & \makecell{1.0(0.27)\\n:1.0(0.30)} & \makecell{0.82(0.33)\\n:0.85(0.33)} & \makecell{0.9(0.47)\\n:0.94(0.47)} & \makecell{1.0(0.34)\\n:1.0(0.36)} & \makecell{0.95(0.50)\\n:0.89(0.50)} & \makecell{0.92(0.52)\\n:0.95(0.51)} & \makecell{1.0(0.30)\\n:1.0(0.30)} & \makecell{0.9(0.52)\\n:0.87(0.52)} & \makecell{0.87(0.54)\\n:0.89(0.54)} \\ \midrule
 & 600 & \makecell{1.0(0.22)\\n:1.0(0.25)} & \makecell{0.89(0.27)\\n:0.9(0.27)} & \makecell{0.84(0.39)\\n:0.89(0.38)} & \makecell{1.0(0.28)\\n:1.0(0.29)} & \makecell{0.85(0.41)\\n:0.91(0.41)} & \makecell{0.81(0.42)\\n:0.92(0.42)} & \makecell{1.0(0.24)\\n:1.0(0.25)} & \makecell{0.88(0.42)\\n:0.95(0.42)} & \makecell{0.92(0.45)\\n:0.91(0.45)} \\ \midrule
\cline{1-11}
\multirow[t]{2}{*}{0.08} & 400 & \makecell{1.0(0.27)\\n:1.0(0.30)} & \makecell{0.88(0.33)\\n:0.9(0.33)} & \makecell{0.91(0.47)\\n:0.89(0.47)} & \makecell{1.0(0.34)\\n:1.0(0.36)} & \makecell{0.93(0.50)\\n:0.86(0.50)} & \makecell{0.81(0.52)\\n:0.83(0.51)} & \makecell{1.0(0.29)\\n:1.0(0.31)} & \makecell{0.87(0.52)\\n:0.91(0.51)} & \makecell{0.9(0.54)\\n:0.88(0.54)} \\ \midrule
 & 600 & \makecell{1.0(0.22)\\n:1.0(0.25)} & \makecell{0.91(0.27)\\n:0.85(0.27)} & \makecell{0.94(0.38)\\n:0.92(0.38)} & \makecell{1.0(0.28)\\n:1.0(0.29)} & \makecell{0.91(0.41)\\n:0.84(0.40)} & \makecell{0.89(0.42)\\n:0.94(0.42)} & \makecell{1.0(0.24)\\n:1.0(0.25)} & \makecell{0.91(0.42)\\n:0.93(0.42)} & \makecell{0.96(0.44)\\n:0.96(0.44)} \\ \midrule
\cline{1-11}
\multirow[t]{2}{*}{0.06} & 400 & \makecell{1.0(0.27)\\n:1.0(0.30)} & \makecell{0.84(0.33)\\n:0.87(0.33)} & \makecell{0.92(0.47)\\n:0.95(0.46)} & \makecell{1.0(0.34)\\n:1.0(0.36)} & \makecell{0.88(0.49)\\n:0.86(0.50)} & \makecell{0.9(0.51)\\n:0.86(0.51)} & \makecell{1.0(0.29)\\n:1.0(0.31)} & \makecell{0.92(0.51)\\n:0.93(0.51)} & \makecell{0.89(0.54)\\n:0.95(0.54)} \\ \midrule
 & 600 & \makecell{1.0(0.22)\\n:1.0(0.25)} & \makecell{0.81(0.27)\\n:0.91(0.27)} & \makecell{0.92(0.38)\\n:0.96(0.38)} & \makecell{1.0(0.28)\\n:1.0(0.29)} & \makecell{0.9(0.41)\\n:0.88(0.41)} & \makecell{0.93(0.42)\\n:0.91(0.42)} & \makecell{1.0(0.24)\\n:1.0(0.25)} & \makecell{0.88(0.42)\\n:0.86(0.42)} & \makecell{0.89(0.45)\\n:0.85(0.45)} \\ \midrule
\cline{1-11}
\bottomrule
\end{tabular}
\end{table}

